Technical Report: Asymmetric Mutual Exclusion for RDMA

Coordinating concurrent access to a shared resource using mutual exclusion is a fundamental problem in computation. In this paper, we present a novel approach to mutual exclusion designed specifically for distributed systems leveraging a popular network communication technology, remote direct memory access (RDMA). Our approach enables local processes to avoid using RDMA operations entirely, limits the number of RDMA operations required by remote processes, and guarantees both starvation-freedom and fairness.

==> Asymmetric Mutual Exclusion for RDMA (Arxiv)/tla/qplock.tex <==
\definecolor{boxshade}{gray}{0.85}

\tlatex
\small
\setboolean{shading}{true}
\@x{}\moduleLeftDash\@xx{ {\MODULE} qplock}\moduleRightDash\@xx{}%
\@x{ {\EXTENDS} Integers ,\, Sequences ,\, TLC}%
\@x{ {\CONSTANTS} NumProcesses ,\, InitialBudget}%
\@x{ {\ASSUME} NumProcesses \.{>} 0}%
\@x{ {\ASSUME} InitialBudget \.{>} 0}%
\@x{ NP \.{\defeq} NumProcesses}%
\@x{ B \.{\defeq} InitialBudget}%
\@pvspace{8.0pt}%
\pcalsymbolstrue
\csyntaxfalse
\@x{\@s{8.06} {\p@mmalgorithm} qplock}%
\@x{ {\p@variables}}%
\@x{\@s{16.4}}%
\@y{\@s{0}%
 Global
}%
\@xx{}%
\@x{\@s{16.4} victim\@s{0.30} \.{\in} \{ 1 ,\, 2 \} ,\,}%
\@x{\@s{16.4} cohort \.{=} [ x \.{\in} \{ 1 ,\, 2 \} \.{\mapsto} 0 ] ,\,}%
 \@x{\@s{16.4} descriptor \.{=} [ x \.{\in} ProcSet \.{\mapsto} [ budget
 \.{\mapsto} \.{-} 1 ,\, next \.{\mapsto} 0 ] ] ,\,}%
\@x{\@s{16.4}}%
\@y{\@s{0}%
 Process-local
}%
\@xx{}%
\@x{\@s{16.4} passed \.{=} [ x \.{\in} ProcSet \.{\mapsto} {\FALSE} ] ,\,}%
\@pvspace{8.0pt}%
\@x{ {\p@define}}%
\@x{\@s{16.4} Us ( pid ) \.{\defeq} ( pid \.{\%} 2 ) \.{+} 1}%
\@x{\@s{16.4} Them ( pid ) \.{\defeq} ( ( pid \.{+} 1 ) \.{\%} 2 ) \.{+} 1}%
\@x{\@s{16.4} Budget ( pid ) \.{\defeq} descriptor [ pid ] . budget}%
\@x{ {\p@end} {\p@define} {\p@semicolon}}%
\@pvspace{8.0pt}%
\@x{ {\p@procedure} AcquireGlobal ( )}%
\@x{ {\p@begin}}%
\@x{\@s{16.4} g1\@s{.5}\textrm{:}\@s{3} victim \.{:=} self {\p@semicolon}}%
\@x{\@s{16.4} gwait\@s{.5}\textrm{:}\@s{3} {\p@while} {\TRUE} {\p@do}}%
 \@x{\@s{50.47} g2\@s{.5}\textrm{:}\@s{3} {\p@if} cohort [ Them ( self ) ]
 \.{=} 0 {\p@then}}%
\@x{\@s{81.87} {\p@goto} g4 {\p@semicolon}}%
\@x{\@s{67.23} {\p@end} {\p@if} {\p@semicolon}}%
 \@x{\@s{50.47} g3\@s{.5}\textrm{:}\@s{3} {\p@if} victim \.{\neq} self
 {\p@then}}%
\@x{\@s{81.87} {\p@goto} g4 {\p@semicolon}}%
\@x{\@s{67.23} {\p@end} {\p@if} {\p@semicolon}}%
\@x{\@s{33.16} {\p@end} {\p@while} {\p@semicolon}}%
\@x{\@s{16.4} g4\@s{.5}\textrm{:}\@s{3} {\p@return}}%
\@x{ {\p@end} {\p@procedure} {\p@semicolon}}%
\@pvspace{8.0pt}%
\@x{ {\p@procedure} AcquireCohort ( )}%
\@x{ {\p@variables} pred}%
\@x{ {\p@begin}}%
 \@x{\@s{16.4} c1\@s{.5}\textrm{:}\@s{3} descriptor [ self ] \.{:=} [ budget
 \.{\mapsto} \.{-} 1 ,\, next \.{\mapsto} 0 ] {\p@semicolon}}%
 \@x{\@s{16.4} swap\@s{.5}\textrm{:}\@s{3} pred \.{:=} cohort [ Us ( self ) ]
 {\p@semicolon} cohort [ Us ( self ) ] \.{:=} self {\p@semicolon}}%
 \@x{\@s{16.4} cwait\@s{.5}\textrm{:}\@s{3}\@s{1.99} {\p@if} {\lnot} ( pred
 \.{=} 0 ) {\p@then}}%
 \@x{\@s{32.8} c2\@s{.5}\textrm{:}\@s{3}\@s{3.22} descriptor [ pred ] . next
 \.{:=} self {\p@semicolon}}%
 \@x{\@s{32.8} c3\@s{.5}\textrm{:}\@s{3}\@s{3.22} {\p@await} Budget ( self )
 \.{\geq} 0 {\p@semicolon}}%
 \@x{\@s{32.8} c4\@s{.5}\textrm{:}\@s{3}\@s{3.22} {\p@if} Budget ( self )
 \.{=} 0 {\p@then}}%
 \@x{\@s{67.10} c5\@s{.5}\textrm{:}\@s{3} {\p@call} AcquireGlobal ( )
 {\p@semicolon}}%
 \@x{\@s{67.10} c6\@s{.5}\textrm{:}\@s{3} descriptor [ self ] . budget \.{:=}
 B {\p@semicolon}}%
\@x{\@s{52.46} {\p@end} {\p@if} {\p@semicolon}}%
 \@x{\@s{32.8} c7\@s{.5}\textrm{:}\@s{3}\@s{3.22} passed [ self ] \.{:=}
 {\TRUE} {\p@semicolon}}%
\@x{\@s{16.4} {\p@else}}%
 \@x{\@s{32.8} c8\@s{.5}\textrm{:}\@s{3} descriptor [ self ] . budget \.{:=} B
 {\p@semicolon}}%
 \@x{\@s{32.8} c9\@s{.5}\textrm{:}\@s{3} passed [ self ] \.{:=} {\FALSE}
 {\p@semicolon}}%
\@x{\@s{16.4} {\p@end} {\p@if} {\p@semicolon}}%
\@x{\@s{16.4} c10\@s{.5}\textrm{:}\@s{3}\@s{4.53} {\p@return} {\p@semicolon}}%
\@x{ {\p@end} {\p@procedure} {\p@semicolon}}%
\@pvspace{8.0pt}%
\@x{ {\p@procedure} ReleaseCohort ( )}%
\@x{ {\p@variables} size ,\, next}%
\@x{ {\p@begin}}%
 \@x{\@s{16.4} cas\@s{.5}\textrm{:}\@s{3} {\p@if} cohort [ Us ( self ) ] \.{=}
 self {\p@then}}%
\@x{\@s{32.8} cohort [ Us ( self ) ] \.{:=} 0 {\p@semicolon}}%
\@x{\@s{16.4} {\p@else}}%
 \@x{\@s{32.8} r1\@s{.5}\textrm{:}\@s{3} {\p@await} {\lnot} ( descriptor [
 self ] . next \.{=} 0 ) {\p@semicolon}}%
 \@x{\@s{32.8} r2\@s{.5}\textrm{:}\@s{3} descriptor [ descriptor [ self ] .
 next ] . budget \.{:=} Budget ( self ) \.{-} 1 {\p@semicolon}}%
\@x{\@s{16.4} {\p@end} {\p@if} {\p@semicolon}}%
\@x{\@s{16.4} r3\@s{.5}\textrm{:}\@s{3}\@s{5.31} {\p@return} {\p@semicolon}}%
\@x{ {\p@end} {\p@procedure} {\p@semicolon}}%
\@pvspace{8.0pt}%
\@x{ {\p@fair} {\p@process} p \.{\in} 1 \.{\dotdot} NP}%
\@x{ {\p@begin}}%
\@x{\@s{16.4} p1\@s{.5}\textrm{:}\@s{3} {\p@while} {\TRUE} {\p@do}}%
\@x{\@s{33.42}}%
\@y{\@s{0}%
 Non-critical section
}%
\@xx{}%
\@x{\@s{33.42} ncs\@s{.5}\textrm{:-}\@s{3} {\p@skip} {\p@semicolon}}%
\@pvspace{8.0pt}%
\@x{\@s{33.42}}%
\@y{\@s{0}%
 Acquire the cohort lock
}%
\@xx{}%
 \@x{\@s{33.42} enter\@s{.5}\textrm{:}\@s{3} {\p@call} AcquireCohort ( )
 {\p@semicolon}}%
\@pvspace{8.0pt}%
\@x{\@s{33.42}}%
\@y{\@s{0}%
 Acquire the global lock, maybe
}%
\@xx{}%
 \@x{\@s{33.42} p2\@s{.5}\textrm{:}\@s{3} {\p@if} {\lnot} passed [ self ]
 {\p@then}}%
\@x{\@s{67.64} {\p@call} AcquireGlobal ( ) {\p@semicolon}}%
\@x{\@s{50.44} {\p@end} {\p@if} {\p@semicolon}}%
\@pvspace{8.0pt}%
\@x{\@s{33.42}}%
\@y{\@s{0}%
 Critical section
}%
\@xx{}%
\@x{\@s{33.42} cs\@s{.5}\textrm{:}\@s{3} {\p@skip} {\p@semicolon}}%
\@pvspace{8.0pt}%
\@x{\@s{33.42}}%
\@y{\@s{0}%
 Release the cohort lock
}%
\@xx{}%
 \@x{\@s{33.42} exit\@s{.5}\textrm{:}\@s{3} {\p@call} ReleaseCohort ( )
 {\p@semicolon}}%
\@x{\@s{16.4} {\p@end} {\p@while} {\p@semicolon}}%
\@x{ {\p@end} {\p@process} {\p@semicolon}}%
\@x{ {\p@end} {\p@algorithm}}%
\@y{%
 ;
}%
\@xx{}%
\pcalshadingfalse \pcalsymbolsfalse
\@pvspace{8.0pt}%
\@x{}%
\@y{\@s{0}%
 Safety
}%
\@xx{}%
 \@x{ MutualExclusion \.{\defeq} ( \A\, i ,\, k \.{\in} ProcSet \.{:} ( i
 \.{\neq} k ) \.{\implies} {\lnot} ( pc [ i ] \.{=}\@w{cs} \.{\land} pc [ k ]
 \.{=}\@w{cs} ) )}%
\@pvspace{8.0pt}%
\@x{}%
\@y{\@s{0}%
 Liveness
}%
\@xx{}%
 \@x{ ExecsCriticalSectionInfinitelyOften \.{\defeq} \A\, i \.{\in} ProcSet
 \.{:} {\Box} {\Diamond} ( pc [ i ] \.{=}\@w{cs} )}%
 \@x{ StarvationFree \.{\defeq} \A\, i \.{\in} ProcSet \.{:} ( pc [ i
 ]\@s{9.22} \.{=}\@w{enter} ) \.{\leadsto} ( pc [ i ] \.{=}\@w{cs} )}%
 \@x{ DeadAndLivelockFree \.{\defeq} ( \E\, i \.{\in} ProcSet \.{:} pc [ i ]
 \.{=}\@w{enter} ) \.{\leadsto} ( \E\, i \.{\in} ProcSet \.{:} pc [ i ]
 \.{=}\@w{cs} )}%
\@pvspace{8.0pt}%
\@x{}%
\@y{\@s{0}%
 Fairness
}%
\@xx{}%
 \@x{ CohortFairness \.{\defeq} \A\, i ,\, j \.{\in} ProcSet \.{:} ( pc [ i ]
 \.{=}\@w{cwait}\@s{0.55} \.{\land} pc [ j ] \.{=}\@w{enter} ) \.{\implies} (
 pc [ i ] \.{=}\@w{cs} \.{\leadsto} pc [ j ] \.{=}\@w{cs} )}%
 \@x{ GlobalFairness\@s{2.86} \.{\defeq} \A\, i ,\, j \.{\in} ProcSet \.{:} (
 pc [ i ] \.{=}\@w{gwait} \.{\land} pc [ j ] \.{=}\@w{enter} ) \.{\implies} (
 pc [ i ] \.{=}\@w{cs} \.{\leadsto} pc [ j ] \.{=}\@w{cs} )}%
\@x{}\bottombar\@xx{}%
\endtla
